WebQuest: A Benchmark for Multimodal QA on Web Page Sequences

The rise of powerful multimodal LLMs has enhanced the viability of building web agents which can, with increasing levels of autonomy, assist users to retrieve information and complete tasks on various human-computer interfaces. It is hence necessary to build challenging benchmarks that span a wide-variety of use cases reflecting real-world usage. In this work, we present WebQuest, a multi-page question-answering dataset that requires reasoning across multiple related web pages. In contrast to existing UI benchmarks that focus on multi-step web navigation and task completion, our dataset evaluates information extraction, multimodal retrieval and composition of information from many web pages. WebQuest includes three question categories: single-screen QA, multi-screen QA, and QA based on navigation traces. We evaluate leading proprietary multimodal models like GPT-4V, Gemini Flash, Claude 3, and open source models like InstructBLIP, PaliGemma on our dataset, revealing a significant gap between single-screen and multi-screen reasoning. Finally, we investigate inference time techniques like Chain-of-Thought prompting to improve model capabilities on multi-screen reasoning.

==> 01_introduction.tex <==
\section{Introduction}
\label{sec:intro}
\todo{jdchen: last pass}
\todo{jasonjlin: done}


\begin{figure*}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/WebQuest_example_skin_care_multi_page.pdf}
    \caption{An example of multi-page question and answering in WebQuest. In this examples, there are 3 screenshots and 2 question-answer pairs. It requires information extraction from each screenshots and reasoning in order to answer both questions. Notice the layouts and font sizes vary among them, as each product is from a different shop.}
    \label{fig:example_of_multi_page_webquest}
\end{figure*}

\noindent As the de facto I/O for Human-Computer Interaction, Graphical User-Interfaces (UIs) allow users to acquire information and complete tasks similar to APIs, as the native interface between computer software.\todo{between software and what? And what is the word software here referring to?}  
A predominant type of data we consume  
are multimodal web pages rich in semantic knowledge and structure. 
The advent of smart devices has promised humans the ease of use, motivating research for multimodal, assistive, predictive, automatic and personalized technology for smart UIs.
However, designers of such systems do not always consider that the Internet is modeled after our cognitive patterns, such as a limited attention span and working memory. Bounded by single-page interfaces and the ability to traverse back and forward in a sequence, machine learning techniques proposed for UI automation are limited in success on multi-step, multi-screen settings, making them unable to fulfill sophisticated tasks for users. Additionally, there are very few datasets focused on information extraction across navigation traces versus task completion.
\\

\noindent Recently, Multimodal Large Language Models (MLLMs) like Gemini \cite{team2023gemini}, GPT-4V \cite{openai2024gpt4} have been trained on text and image data crawled from the web to demonstrate powerful zero shot capabilities.
However, the data collection process of visual-language datasets~\cite{schuhmann2021laion400m,schuhmann2022laionb} 
reveals a discrepancy with how a human user would interact with the web: navigating \textit{multiple pages} searching for information using %
the various UI elements present on the UI. By simply extracting text and images from web pages, these datasets not only remove the functional congruence shared between desktop and mobile form factors, but also fail to capture the actions taken and the implicit retrieval requirement that is common to a information-seeking or goal-oriented workflow, i.e. flight booking or shopping. As a result, these models are effective in general reasoning, but perform poorly when used as end-to-end autonomous agents.
\\

\noindent A key challenge in developing UI agents is that they not only have to interpret spatial relations between structures, they also have to ground open ended instructions within an expanding set of semantically correlated pages across diverse applications.
Traditional NLP benchmarks like question answering (QA) and information retrieval have been adapted for visual grounding, but they contain either single-page or multi-page questions that contain the answer on one of the pages. We postulate the lack of a temporal dimension might stem from human's limited working memory and the limitations of existing models to effectively predict such complex interactions. %
When provided a sequence of pages, local similarity between adjacent pages requires a model to discern relevant information among confounding concepts.
It can therefore be limiting to develop and evaluate LLM agents using only the standard QA formulation. To this end, we modify the QA formulation to include multiple pages, which more accurately reflects a user's ability to compare and reason across pages, i.e. \textit{``If I restrict the take-off time to be between 8:00 AM and 8:00 PM, how much more I need to pay for the best choice in business class?''}\todo{sri: Make the example here consistent with the figure. Also explain a little bit more why this is needed.}
to arrive at an informed decision or conclusion. We do acknowledge that some sophisticated websites already provide filters and comparison functionalities, but they are limited to popular options and do not always expose all the functionality available to the user. %

\noindent Motivated by this question, %
we introduce WebQuest, a multi-page screen question-answering dataset, to emulate both navigation and retrieval reasoning settings formulated as a VQA evaluation of multimodal web agents. The dataset and related code will be released on github at: <to-be-updated>.  Figure~\ref{fig:example_of_multi_page_webquest} illustrates an example of multi-screen question answering. We seek to close the gap between general QA-based content understanding and agent model research by providing a novel mode of QA setting. Our dataset targets question-answering across web interaction sequences grounded in real world user behavior. WebQuest includes three question categories: single-screen QA, multi-screen QA, and QA on navigation traces. The first two involve multimodal content from one or more screens, while navigation trace questions are based on sequences of screens navigated by humans to perform routine tasks. This necessitates the endowment of retrieved knowledge from relevant parts of the sequence to aid with complex screen understanding.
\\
\todo{sri: add a table comparing other datasets for UI related tasks.}

\noindent Finally, we evaluate various state-of-the-art proprietary models GPT-4V~\cite{openai2024gpt4}, Gemini Flash~\cite{geminiteam2024gemini}, Claude 3~\cite{anthropic2024claude3}, and open source models like InstructBLIP~\cite{dai2023instructblip}, PaLIGemma~\cite{beyer2024paligemma} via prompt engineering and Chain-of-thought prompting, revealing a significant gap between single-page and multi-page reasoning. 
 The main contributions of our work are multifold and we believe it will advance the field of UI understanding and automation.
\begin{itemize}
    \item
        WebQuest is the first dataset containing QA over multiple screens and navigation traces requiring information from more than one screen to answer the question. In addition, each multi-screen and trace QA example spans various related websites.\todo{sri:rephrase this while preserving all the info.} 
    \item
        We release 3 subsets of data containing single-screen, multi-screen and navigation traces, enabling more detailed benchmarking of the capabilities of different models.
    \item
        For the trace QA split, we also provide step-by-step supervision for the data which can help improve models on UI navigation for the purpose of answering questions or extracting information.
\end{itemize}



==> a_data_collection_details.tex <==
\section{Data Collection Details}
\subsection{Data Collection Instructions}
The data collection process was performed with human raters who were responsible for capturing the screenshots and generating the corresponding questions and answers. In each task, raters are asked to collect screenshots and QA on a specific website category like Shopping, Restaurants etc. 
For \emph{Single Screen QA}, we give the following instructions to the raters. 
\begin{enumerate}
\item Consider a scenario where a user is viewing a webpage to looking up information regarding shopping, restaurants, and etc. 
\item Capture 1 screenshot taken from Google Chrome (desktop) without signing into any accounts.
\item Generate a question-answer pair focusing on arithmetic or logical reasoning reflecting real world usage.
\end{enumerate}
In contrast to \emph{Single Screen QA}, the \emph{Multi ScreenQA split} focuses on analyzing information across various websites and webpages.
The instructions given to the raters for \emph{Multi Screen QA} are shown below:
\begin{enumerate}
\item Consider use cases where a user is researching a product to buy or comparing options from different web-sites.
\item Capture 3-5 web screenshots taken from Google Chrome (desktop) spanning websites related to each other.
\item Most of these screenshots should be from different websites.
\item Generate a question-answer pair focusing on arithmetic or logical reasoning.
\item Ensure that answering the question needs to use information from all the screenshots.
\end{enumerate}

For the \emph{Trace QA} split, similar to the \emph{Multi Screen QA} split, the raters are asked to focus on specific website category. They are asked to install custom Chrome Extension which enables them to record their interactions on the screen. The chrome extension is meant to be turned on when the rater is ready to collect data. They can pause, review or delete any of the data captured. After collecting the trace, the raters add questions and answers related to the screenshots in the trace. The specific instructions are shown below:
\begin{enumerate}
\item Consider use cases where a user is researching a product to buy or comparing options from different web-sites.
\item Go to the first web page and start the trace recording.
\item Navigate through the different webpages as part of the trace. Once the navigation is complete, click "stop" on the recording and review the screenshots captured.
\item Delete any screenshots containing any personal information.
\item Generate a question-answer pair focusing on arithmetic or logical reasoning.
\item Ensure that answering the question needs to use information from about 3-5 screenshots.
\end{enumerate}

\subsection{Rater Details}
For the \emph{Multi Screen QA} task, we used 10 raters with ages between 25 and 35 based in India. The raters were employed as contractors to help with various data collection tasks apart from this task.

For the \emph{Trace QA} task, the authors of the paper collected the data. They are based in the United States and Europe.


==> acknowledgments.tex <==
\section*{Acknowledgments}

We thank ....\todo{To be complete in camera-ready version}

